Fake News Detection on Social Media using Geometric Deep Learning

Social media are nowadays one of the main news sources for millions of people around the globe due to their low cost, easy access and rapid dissemination. This however comes at the cost of dubious trustworthiness and significant risk of exposure to 'fake news', intentionally written to mislead the readers. Automatically detecting fake news poses challenges that defy existing content-based analysis approaches. One of the main reasons is that often the interpretation of the news requires the knowledge of political or social context or 'common sense', which current NLP algorithms are still missing. Recent studies have shown that fake and real news spread differently on social media, forming propagation patterns that could be harnessed for the automatic fake news detection. Propagation-based approaches have multiple advantages compared to their content-based counterparts, among which is language independence and better resilience to adversarial attacks. In this paper we show a novel automatic fake news detection model based on geometric deep learning. The underlying core algorithms are a generalization of classical CNNs to graphs, allowing the fusion of heterogeneous data such as content, user profile and activity, social graph, and news propagation. Our model was trained and tested on news stories, verified by professional fact-checking organizations, that were spread on Twitter. Our experiments indicate that social network structure and propagation are important features allowing highly accurate (92.7% ROC AUC) fake news detection. Second, we observe that fake news can be reliably detected at an early stage, after just a few hours of propagation. Third, we test the aging of our model on training and testing data separated in time. Our results point to the promise of propagation-based approaches for fake news detection as an alternative or complementary strategy to content-based approaches.

==> sections/related.tex <==
\section{Related work}


social bots play a key role in spreading fake news \cite{shao2017spread}



user profile to determing users more succeptible to fake news \cite{shu2018understanding}

==> sections/results.tex <==


\section{Results}
\label{sec:results}


We considered two different settings of fake news detection: {\em URL-wise} and {\em cascade-wise}, using the same architecture for both settings. In the first setting, we attempted to predict the true/fake label of a URL containing a news story from all the Twitter cascades it generated. On average, each URL resulted in approximately 141 cascades. 
%
In the latter setting, which is significantly more challenging, we assumed to be given only one cascade arising from a URL and attempted to predict the URL label. Our assumption is that all the cascades associated with a URL inherit the label of that URL. While we checked this assumption to be true in most cases in our dataset, it is possible that an article is e.g. tweeted with a comment denying its content. 
%
We leave the analysis of comments accompanying tweets/retweets as a future research direction. 




\begin{figure}[t]
    \centering
    \setlength\figureheight{6cm}
    \setlength\figurewidth{1.0\linewidth}
    \input{figures/combined_roc.tex}%figures/roc_5fold_24h.tikz}
    \caption{Performance of URL-wise (blue) and cascade-wise (red) fake news detection using 24hr-long diffusion time. Shown are ROC curves averaged on five folds (the shaded areas represent the standard deviations). ROC AUC is 92.70 $\pm$ 1.80\% for URL-wise classification and 88.30 $\pm$ 2.74\% for cascade-wise classification, respectively. Only cascades with at least 6 tweets were considered for cascade-wise classification.}
    \label{fig:roc_24h_5_folds}
\end{figure}





\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/tsne_embedding_all_nodes.png}
%    \includegraphics[width=1.0\linewidth]{figures/pca_embedding_all_nodes.png}
    
    \caption{T-SNE (top) %and PCA (bottom) 
    embedding of the vertex-wise features produced by our neural network at the last convolutional layer representing all the users in our study, color-coded according to their credibility (blue = reliable, red = unreliable). Clusters of users with different credibility clearly emerge, indicative that the neural network learns features useful for fake news detection.}
    \label{fig:t-sne-embedding}
\end{figure}



\subsection{URL-wise fake news classification}

\begin{figure}[t]
    \centering
    
    \setlength\figureheight{5.5cm}
    \setlength\figurewidth{1.0\linewidth}
    \begin{minipage}{1.0\linewidth}
    \input{figures/diffusion_5folds_up_to_24h.tikz}
    \end{minipage}\vspace{2mm}
    \begin{minipage}{1.0\linewidth}
    \input{figures/cascade_diffusion_5folds_up_to_24h_min_no_tweets=6_max_val_roc_auc.tikz}
    \end{minipage}
    \caption{Performance of URL-wise (top) and cascade-wise (bottom) fake news detection (mean ROC AUC, averaged on five folds) as function of cascade diffusion time.}
    \label{fig:diffusion_roc_auc_24h_5_folds}
\end{figure}

\begin{figure}[t]
    \centering
    \setlength\figureheight{5cm}
    \setlength\figurewidth{1.0\linewidth}
    \begin{minipage}{1.0\linewidth}
    \input{figures/reverse_ablation_test_AUC.tikz}
    \end{minipage} \vspace{2mm}
    \hfill
    \begin{minipage}{1.0\linewidth}
    \setlength\figurewidth{1.0\linewidth}
    \input{figures/reverse_ablation_cascadewise_min6_max_val_AUC_test_AUC.tikz}
    \end{minipage}
    \caption{Ablation study result on URL-wise (top) / cascade-wise (bottom) fake news detection, using backward feature selection. Shown is performance (ROC AUC) for VeritasZero trained on subsets of features, grouped into four categories: user profile, network and spreading, content, and user activity. Groups are sorted for importance from left to right.%: user profile (??), network and spreading (social graph, retweet cascades and timestamps), content (word embedding of the tweet), and user activity (??).
    }
    \label{fig:ablation_study}
\end{figure}

\label{sec:url-class}

%We begin our experimental evaluation with URL-wise classification. 
% Given a specific URL $u$ with corresponding tweets $T_u = \{t_u^1, t_u^2,..., t_u^N\}$ mentioning it, we describe $u$ by means of the associated sub-graph $G_u$ induced from Twitter's network. Every node of $G_u$ corresponds to a tweet/retweet and is represented by both user and tweet related features. Two nodes $i$ and $j$ are connected by two directed edges $ij$ (from $j$ to $i$) and $ji$ (from $i$ to $j$) if at least one of the two corresponding users follows the other ($G_u$ is an undirected graph). A one-hot encoding for each possible \emph{following} relation (i.e. $i \leftarrow j$, $j \leftarrow i$) has been used to characterize the three types of possible social connections (i.e. $i \leftarrow j$, $i \rightarrow j$, $i \leftrightarrow j$).
% Each relation has been encoded according to a one-hot encoding scheme.
%A one-hot encoding describing the direction of the following relationship has been used to characterize different types of social connections i.e. $i \leftarrow j$, $i \rightarrow j$, $i \leftrightarrow j$. 
% This particular configuration allows to spread information independently by the directions of the relations while potentially giving different importance to the types of connections. $ij$ features are concatenated to the ones of nodes $i$, $j$ in the attention projection layer to achieve such behavior. Section \ref{sec:input-feat} presents the set of features exploited for describing the different nodes.
% The pre-trained version of Glove\footnote{\url{https://nlp.stanford.edu/projects/glove/}} \cite{} for Twitter has been used for describing the content of the tweets and the descriptions of the users in input to the model.
% With the aim of providing a challenging problem to the NN, only tweets and retweets posted in the first day of a generic URL $u$'s life are used to construct $G_u$ (if $u$ appears on Twitter at time $t$, only tweets/retweets published in $[t, t+24h]$ are fed in input to the model). Figure \ref{fig:roc_24h_5_folds} presents the performance achieved by our GCNN after 24h. 5 folds cross-validation has been used in our experiments to reduce the bias of the estimation while containing the overall computational cost. VeritasZero achieves an average ROC AUC equal to 92.70 $\pm$ 1.80\% on such experiment.

{\bf Diffusion performance.} One of the key characteristics a fake news detector must present is speed. As our approach relies on the diffusion of news on social networks, we decided to investigate the performance of VeritasZero by classifying the provided URLs after multiple hours of diffusion on Twitter. Provided a generic URL $u$ and a diffusion time $d$, we classify $u$ by processing its corresponding $G_u^d$ induced subgraph where only tweets/retweets published in $[t, t+d]$ are used as vertices. %With the aim of providing a challenging problem to the NN, we decided to analyze multiple diffusion times in just the first 24hrs of life of a URL on Twitter. 
Figure \ref{fig:diffusion_roc_auc_24h_5_folds} - top highlights the performance achieved by VeritasZero for multiple $d$ within 24 hours.
5 folds cross-validation has been used to reduce the bias of the estimations while containing the overall computational cost. %We limited ourselves to the first 24hrs of a tweet life to provide a challenging problem to the model. 
As one may expect, performance shows an increasing trend in time which roughly saturates after 15hrs. At 0hrs the performance of the model without diffusion (i.e. with just the first tweet mentioning the URL) is shown. Figure \ref{fig:roc_24h_5_folds} details the performance of our model at the maximum considered diffusion time. At 24 hours, VeritasZero achieves an average ROC AUC equal to 92.70 $\pm$ 1.80\%. Figure \ref{fig:t-sne-embedding} shows an average embedding for each user in the dataset, according to the vertex-wise features produced by the last convolutional layer. Clusters of different tweeters appear in the embedding space with a relatively clear separation between reliable and unreliable users.


{\bf Aging.} In the previous subsection we analyzed the performance of our model on a typical offline classification task, where all the news is gathered and comes from a variety of past instants of time. In this subsection we investigate the performance of VeritasZero on an online classification problem where only URLs published in the past are available at training time and the model has to predict the veracity of URLs coming from the future. Due to the continuously evolving state of the world, we argue that such task is more challenging for a generic content-based classifier, as the veracity of a given piece of news intrinsically depends on the political/social context of the world at publication time. %availableevents occurring at publication time.
%However, a classic use-case for fake n to A typical use-case for VeritasZero is to predict the veracity of future news gathered from the considered social media  
%In order to assess the capability of VeritasZero to predict the veracity of future news while being trained only on past ones, we performed an aging-study on the proposed model.
In order to assess the capability of VeritasZero on such setting, we split the considered dataset in two subsets of news: training-validation (80\% of urls) and testing (20\% of urls). The two subsets are completely disjoint and subsequent in time (i.e. the mean dates of the training and validation sets are in August 2016, while the one for the test set is December 2016).
We assessed the results of our model on multiple, partially overlapping time windows which appear one after another in the test set. Each window is at least 20\% the size of the test set and the average dates of two consecutive windows are at least 14 days apart. Figure \ref{fig:aging_url} highlights the variation in performance due to aging of the training set.
%We then performed multiple tests on different test sliding-windows of times of the test sets, the performance obtained by our model are reported in Figure \ref{fig:aging_url}.
VeritasZero exhibits a slight deterioration in performance only after 190 days, likely because of the different behavior of far apart news. 
%VeritasZero shows a slight deterioration in performance only after 190 days, likely because of the different behavior exhibited by news distant in time w.r.t. those the model have been trained on.

% dataset statistics:
% [i] URL distribution:
% Total: 1129
% Training: 677 (0.60)
% Validation: 226 (0.20)
% Test: 226 (0.20)

% [i] Veracity (T/F ratio):
% Total: 4.97
% Training: 6.44
% Validation: 6.53
% Test: 2.32

% Average tweets per URL (all): 535.01
% Average tweets per URL (train): 374.09
% Average tweets per URL (val): 386.72
% Average tweets per URL (test): 1165.36

% [i] Dates distribution ( | min -- avg -- max | ):
% Training:   | 2013-05-04 -- (2016-08-05) -- 2016-09-27 |
% Validation: | 2014-09-23 -- (2016-08-07) -- 2016-09-27 |
% Test:       | 2016-09-27 -- (2016-12-11) -- 2018-01-29 |

{\bf Ablation study.} To finally highlight the importance of the different categories of features provided in input to the model, we conducted an ablation study by means of backward-feature selection. % (Section \ref{sec:groups-feat} details the groups we constructed). 
Figure \ref{fig:ablation_study} shows the results of such experiment. User-profile and network/spreading appear as the two most relevant groups for achieving satisfactory results with the proposed model (average ROC AUC $\geq$ 90\%).


\subsection{Cascade-wise fake news classification}

\begin{figure}[t]
    % \setlength\figureheight{8cm}
    % \setlength\figurewidth{12cm}
    % \input{figures/aging_uw_mean.tikz}
    \setlength\figureheight{5.5cm} %5.5cm
    \setlength\figurewidth{1.0\linewidth}  %7.3cm
    \begin{minipage}{1.0\linewidth}
    %\hspace*{-5mm}
    \centering
    \input{figures/aging_uw_mean.tikz}
    \end{minipage}
    \begin{minipage}{1.0\linewidth}
    \centering
    \input{figures/aging_cw_cw_mean.tikz}
    \end{minipage}
    \caption{Effects of training set aging on 
    URL-wise (top) / cascade-wise (bottom) fake news detection with VeritasZero. Horizontal axis shows difference in days between average date of the training and test sets. Shown is the test performance obtained by our model 
    with 24hrs diffusion (solid blue), test performance obtained with same model just using the first tweet of each piece of news (0hrs diffusion, dashed orange), and test performance obtained training on our original uniformly sampled five folds (veracity predictions are computed for each URL/cascade when this appears as a test sample in our 24hrs five fold cross-validation, green).}
    %training our model on past URLs and testing on multiple future windows of time . In green, test performance obtained training on our original uniformly sampled 5 folds and testing on same windows of time (veracity predictions are computed for each URL when this appears as a test sample in our 24hr 5 fold cross-validation).}
    \label{fig:aging_url}
\end{figure}

\label{sec:cascade-class}


\begin{figure}[t]
    \setlength\figureheight{5.5cm}
    \setlength\figurewidth{1.0\linewidth}
    \begin{minipage}{1.0\linewidth}
    \centering
    \input{figures/cascade_mean_roc_auc_5folds_up_to_24h_multi_min_no_tweets.tikz}
    \end{minipage}
    \caption{Performance of cascade-wise fake news detection (mean ROC AUC, averaged on five folds) using minimum cascade size threshold. Best performance is obtained by filtering out cascades smaller than 6 tweets. }
    %\caption{Distribution of cascades over the 930 URLs available in our dataset with at least 6 tweets per cascade. The first 15 URLs (\char`\~1.5\%)  represent 20\% of all the available cascades.}
    \label{fig:cw-min-thresh}
\end{figure}




%As illustrated in Section \ref{}, 
%Fake-news may exist at different levels on social-media: a piece of news may try to mislead readers by distorting reality and presenting false statements, or people (in our case, tweeters) may take true pieces of news and deceive fellow users by misrepresenting these with false comments. % about the content of the article at hand. 
%Because of this, 
%To verify the capabilities of our model in classifying fake-news at multiple levels, 
%For this reason, we decided to detect fake news at a tweet-level by classifying the veracity of the single cascades which may be associated to a given URL.
%we decided to further analyze the single cascades which may arise from a given URL. For simplicity, we assumed that the veracity of every single cascade in this problem corresponds with the one of the associated URL (independently by the content of the tweet). This clearly sub-optimal choice allowed us to extend the labels of the URLs to single tweets, providing a considerably large dataset of cascades (159,652 samples) without any further annotation process. We leave to future research a second analysis of this problem with proper cascade-wise labels. %, avoiding any second annotation process in our experiments.

{\bf Performance for multiple cascade sizes.} %Differently from URLs, single cascades may present a relatively small number of (re)tweets on Twitter. 
%Differently from URLs,
%Because of their local nature, 
Because of their localized nature, single cascades may easily present a small amount of (re)tweets if produced by users with limited number of followers. Since our solution relies however on the spreading of information among people, such examples may be hard to classify as no clear diffusion pattern may easily emerge in the considered social graph. %Figure \ref{fig:cw-min-thresh} shows the performance of VeritasZero for cascades of multiple minimum sizes. As one may expected, the model improves in performance with larger cascades reaching saturation for cascades of at least 6 tweets (5,976 samples). thanks to the larger amount of available data and richer patterns this can detect. 
To identify the minimum number of (re)tweets a cascade should present for producing good performance with our model, we investigated the performance of VeritasZero on cascades of multiple minimum sizes (Figure \ref{fig:cw-min-thresh}).
%in the we decided to investigate the performance of VeritasZero on cascades of multiple minimum sizes. The purpose of this analysis is to find minimum number of (re)tweets a cascade should present to guarantee good performance with our model at test time. The results of this analysis are depicted in Figure \ref{fig:cw-min-thresh}.
%such small cascades may be hard to classify present excessively poor diffusion patterns to guarantee good performance with our model. To thus identify the minimum cascade-size that guarantees good performance with our model, we decided to investigate the performance of VeritasZero on cascades of multiple minimum sizes (Figure \ref{fig:cw-min-thresh}).
%As our solution relies on the spreading of information among people, we decided to investigate as first task the performance of 
%As our solution is based on diffusion, we investigated the performance of VeritasZero for cascade-wise classification on cascades of multiple minimum sizes. The main idea is to find a reasonable minimum cascade size that allows to identify sufficiently rich diffusion patterns for guaranteeing good performance with our model. 
%The results of this analysis are depicted in Figure \ref{fig:cw-min-thresh-and-URLs-distribution-cw-ds}-top. 
Only cascades of at least 3 tweets have been considered, as they represent the smallest cascades with a non-trivial diffusion pattern one can have. As expected, the model improves in performance with larger cascades, reaching saturation for cascades of at least 6 tweets (5,976 samples). % Only cascades with at least 6 tweets has been considered for all the experiments illustrated in the next subsections

To provide meaningful data in input to our model, in subsequent experiments we considered such cascade size as the minimum acceptance threshold for VeritasZero (i.e. no cascade with less than 6 tweets has been processed with our model in the remainder of this section).%, in order to guarantee meaningful samples in input to the model.% samples with sufficiently rich spreading patterns.  %Because of this, only cascades of at least 6 tweets will be considered in the next subsections.

{\bf Ablation study.} %Fixed the minimum size of the cascades provided in input to VeritasZero, 
To validate the importance of all features at cascade-level, we performed a second ablation study for cascade-wise classification. Interestingly, while all features were positively contributing to the final predictions at URL-level, removing tweet content from the provided input improves performance of 4\% at cascade-level. This apparently contradicting result can be explained by looking at the distribution of cascades over all the available URLs (Figure \ref{fig:URLs-distribution-cw-ds}): 20\% of cascades are associated to the top 15 largest URLs (out of 930) in our dataset (\char`\~1.5\%). Since tweets citing the same URL typically present similar content, it is easy for the model to overfit on this particular feature. Proper regularization (e.g. dropout, weight decay) should thus be introduced to avoid overfitting and improve performance at test time. %To highlight however the capabilities of our model to classify fake-news in a content-free scenario, 
For simplicity, by leveraging the capabilities of our model to classify fake-news in a content-free scenario, we decided to completely ignore content-based descriptors for cascade-wise classification (i.e. we let the model exploit only users-/diffusion-related features to solve cascade-wise classification). %We leave to future works a proper estimation of a dropout rate to use for maximizing performance on this particular task. %We argue that similar results to the ones illustrated in the next sub-subsections can be achieved for URL classification, as performance drops only of \char`\~3\% when content-based descriptors are removed on this particular task (Figure \ref{fig:ablation_study}-top). % in our next experiments. 


{\bf Diffusion performance.} Following what presented in Section \ref{sec:url-class}, we repeated our diffusion experiment for cascade-wise classification (Figure \ref{fig:diffusion_roc_auc_24h_5_folds}-bottom). As expected, our model improves with time due to the richer patterns that emerge with diffusion. Differently from what observed in the previous section, however, the model converges more quickly for cascade-wise classification and saturates already after just 7 hours of diffusion. This different behavior is mainly due to the simpler topological patterns and shorter life cascades shown on Twitter. After 7 hours, 81\% of the tweets available in the first day of life of a generic cascade are in this sense produced. Such percentage dramatically drops to 58\% for URLs at the same instant of time. At 15 hours (i.e. at saturation point for URL-wise classification), 82\% of a generic URL tweets are instead available.

%Because indeed of their locality, cascades show on Twitter a much shorter spreading wrt URLs, this effect appears clear comparing the saturations points of both cascades and URLs: after 4hrs of diffusion, cascades already completed 73\% of their spreading while URLs only 43\% at the same instant of time. %  and to the shorter spreading cascades show on Twitter, 

{\bf Aging.} As we did for URL-wise classification (see Section \ref{sec:url-class}), we investigated the performance of our model wrt aging of the training set, i.e. 
we evaluated VeritasZero on multiple future windows of time while training on the past. Both the split between training-validation and test sets and the generation of the time windows have been performed similarly to the URL-based experiment (80\% vs 20\%, average dates respectively in August 2016 and February 2017, time windows at least 20\% of the test set size and at least 14 days apart). 
% in addition, === add details about the parallel split between snopes and buzzfeed?
The performance of our model over time is illustrated in Figure \ref{fig:aging_url}-bottom. VeritasZero shows in this case a more robust behavior wrt URL-classification, losing only 4\% between 60 and 260 days. % slightly decreasing only at first and then reaching a pleateau around 130 days.
This different behavior is likely due to the higher variability that characterizes cascades as opposed to URLs. %being these represented by small and simpler gr 
As cascades are represented by smaller and simpler graphs, the likelihood of identifying recurrent rich structures between different training samples is lower compared to the URL-case. Our diffusion based model is thus forced to learn simpler and more robust features for classifying the provided samples, as cascades may easily involve sets of really different users coming from really different areas of the Twitter social network. To prove this statement we analyzed the mean average distance\footnote{Provided N cascades/URLs $\{s_1, s_2,\ldots, s_N\}$, we compute the mean average distance between the users of such samples and all the remaining ones as: $MAD = \frac{1}{N}\sum_{t=1}^{N} (\frac{1}{M_t}\sum_{u=1}^{M_t}{d_t^u}$); with $d_t^u$ the distance of user $u$ wrt his/her nearest neighbor in the remaining training samples. \textcolor{red}{DE: What is $M_t$ here? How is the distance calculated?}} users of 100 training cascades/URLs present wrt their corresponding nearest neighbors in the remaining training samples, while for URLs the mean minimum distance is equal to 1.69 $\pm$ 0.849, for cascades it grows up to 2.55 $\pm$ 0.630 (\char`\~51\% higher) implying lower similarities among users of different examples. \textcolor{red}{(FM: I also computed the mean minimum distance ($MMD = \frac{1}{N}\sum_{t=1}^{N} min_u {d_t^u}$) between users, in this case the values are 0.0733 $\pm$ 0.369 for URLs and 0.771 $\pm$ 1.031 for cascades. This is due to the high probability we have of finding one user of one URL in at least an other URL, for cascades this is much less likely as cascades are more localized and may involve sets of really different people (which potentially are unique for the single cascades). I would stay with the mean average distance as it provides an "expected" distance of a generic sample wrt all the other ones and in general it looks less "suspicious" as the distance for URLs is really really low after all (in 96\% of the cases we find in a URL at least a user that we observe in an other sample, for cascades "just" for the 61\% of the cases). Overall, this is suggesting me that the model is actually able to generalize over users it has not seen in the past (as for both cases the \% of users in the test set observed in the training time decreases over time but for cascade-wise classification performance remains constant for some time), but if over 1000 URLs we keep observing the same users, it makes just sense that the model learns a signature of those.)}
%To prove this statement we analyzed the mean minimum distance\footnote{Provided N cascades/URLs $\{s_1, s_2,\ldots, s_N\}$, we compute the mean minimum distance between the users of such samples and all the remaining ones as: $MMD = \frac{1}{N}\sum_{t=1}^{N} min_u {d_t^u}$; with $d_t^u$ the distance of user $u$ wrt his/her nearest neighbor in the remaining training samples.} users of 100 training cascades/URLs present wrt their corresponding nearest neighbors in the remaining training samples, while for URLs the average minimum distance is equal to 0.0733, for cascades it grows up to 0.771 implying lower similarities among users of different examples.% and in general a higher variability of the provided training set. %Thanks to the higher entropy of the provided training data, the final model thus appears more robust towards aging of the training set, while presenting slightly lower performance if compared on a classic uniform split (ROC AUC equal to 88\% vs 93\%).%This particular regularization effect makes the model more robust towards aging of the training 
%naturally produces as result a slightly loss in performance on a classic uniform split, but at the same time allows the model to be more robust towards aging of the training set 
%naturally involves a slightly loss in performance on a uniform split of the data, however at the same time makes the model more robust to aging of the training set 
%the characteristics of the users involved in each of the provided   of users involved in each single sample may highly vary from one case to the other. This  making for the network harder predicting  the provided samples
%As cascades bring less information wrt URLs (being these a sub-portion of URLs themesleves)  Being cascades smaller samples wrt URLs, the users involved in the 
%specific class of cascades we used in our analysis. By limiting ourselves to cascades with at least 6 tweets, we implicitly contained the variability of observed users in our dataset, thus making the aging problem simpler for the considered model (...checking this...).%in our dataset as mostly cascades tweeted/retweeted by big cascades are typically produced by popular users

%simpler topology cascades present wrt URLs, 
%This different behavior is likely due to the smaller size cascades present wrt URLs, which implicitly limits the variability of the available data and the richness of the learned filters (thus improving the robustness of the model wrt aging of the considered training set). {\textcolor{red}{(FM: to rephrase, we also have to mention we used same URL split for previous experiments while here we split again to balance the T/F ratio)}.% This different behavior is likely due to the smaller size cascades present wrt URLs, which implicitly limits the variability of the available data over time and the richness of the realized filters (the final model appears thus simpler and more robust to aging of the considered training set). {\textcolor{red}{(FM: we have to mention we used same URL split for previous experiments while here we split again to balance the T/F ratio)}.
%While VeritasZero degenerates more quickly w.r.t. the URL-case (likely because of the less rich diffusion information cascades show w.r.t. URLs), performance obtained with 24 hours diffusion and within 50 days from the training set still appears close to the one achieved in the uniformly sampled five-folds case. %In addition, Figure \ref{fig:aging_cascades} shows how the same model trained only on the first tweet doesn't perform as well on future windows of time, implying the information extracted from the diffusion of the root-tweet represent a meaningful information for generalizing over time.

% dataset statistics:
% [i] Cascades distribution:
% Total: 5976
% Training: 3585 (0.60)
% Validation: 1195 (0.20)
% Test: 1196 (0.20)

% [i] Veracity (T/F ratio):
% Total: 4.42
% Training: 4.13
% Validation: 4.13
% Test: 5.99

% Average tweets per cascade (all): 50.51
% Average tweets per cascade (train): 39.59
% Average tweets per cascade (val): 39.16
% Average tweets per cascade (test): 94.55

% [i] Dates distribution ( | min -- avg -- max | ):
% Training:   | 2013-05-06 -- (2016-08-22)(2016-09-22) -- 2017-05-18 |
% Validation: | 2013-05-04 -- (2016-08-17)(2016-09-22) -- 2017-05-18 |
% Test:       | 2016-09-27 -- (2017-02-04)(2016-09-28) -- 2018-01-29 |

==> sections/sup_material.tex <==
\section{Supplementary Material}

\subsection{Input features}
\label{sec:input-feat}
user self characterization notext:
   \begin{itemize}
       \item geo enabled user
       \item background picture user
       \item default profile user
       \item default profile image user
       \item lang user
   \end{itemize}

user self characterization text:
    \begin{itemize}
        \item description user
    \end{itemize}

user activity:
    \begin{itemize}
        \item statuses count user
        \item favourites count user
        \item listed count user
    \end{itemize}

user social characterization:
    \begin{itemize}
        \item verified user
        \item followers count user
        \item friends count user
        \item created at user
    \end{itemize}
 
tweet propagation:
    \begin{itemize}
        \item source tweet
        \item time delta tweet
        \item reply count retweeted
        \item quote count retweeted
        \item favorite count retweeted
        \item retweet count retweeted
    \end{itemize}

tweet content:
    \begin{itemize}
        \item text tweet
        \item hashtags tweet
    \end{itemize}
